Skedulix: Hybrid Cloud Scheduling for Cost-Efficient Execution of Serverless Applications

We present a framework for scheduling multifunction serverless applications over a hybrid public-private cloud. A set of serverless jobs is input as a batch, and the objective is to schedule function executions over the hybrid platform to minimize the cost of public cloud use, while completing all jobs by a specified deadline. As this scheduling problem is NP-Hard, we propose a greedy algorithm that dynamically determines both the order and placement of each function execution using predictive models of function execution time and network latencies. We present a prototype implementation of our framework that uses AWS Lambda and OpenFaaS, for the public and private cloud, respectively. We evaluate our prototype in live experiments using a mixture of compute and I/O heavy serverless applications. Our results show that our framework can achieve a speedup in batch processing of up to 1.92 times that of an approach that uses only the private cloud, at 40.5% the cost of an approach that uses only the public cloud.

==> Section_framework-architecture-long.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Framework Architecture}
\begin{figure*}[tpb]
\centering
\begin{subfigure}[b]{0.55\linewidth}
      \centering
      \includegraphics[scale=0.36]{Images/AWS_cloud_edge_framework_Diagram_new}
      \caption{Framework Architecture}      \label{fig:system_architecture}
     \end{subfigure}%
\begin{subfigure}[b]{.4\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{Images/Video_pipeline_DAG.pdf}
%      \caption{A DAG of Video Processing Pipeline.}      \label{fig:videopipeline}
	\centering
    \includegraphics[scale=.4]{Images/scheduler}
    \caption{Scheduler Implementation.} \label{fig:openfaas}
     \end{subfigure}
\caption{Framework architecture and the scheduler implementation on OpenFaaS}
\label{fig.system_architecture_with_scheduler}
\end{figure*}
The framework architecture is shown in Fig.~\ref{fig:system_architecture}. The system consists of a private cloud environment and a public cloud environment. The scheduler also resides in the private cloud. The scheduler contains one subprocess for each stage, as shown in the figure. Jobs consisting of multiple stages arrives at the system via a gateway in a batch, i.e., $J$, jobs arrive at the system at the same time. 
The scheduler intercepts the incoming jobs and dispatches them according to the appropriate schedule using Alg.\ref{alg.main_algorithm}. 

%In Sec.~\ref{experiments.sec}, to compare our approach with optimal, we also execute jobs according to the schedule obtained by solving the MILP in Gurobi (in Eq.~\eqref{objective.eq}-\eqref{xbin.con} in Appendix~\ref{problem.sec}). In this case, the output of the solver is a schedule (generated as a text file), which gives us a start and end time of each job stage (based on the predicted execution times described in Sec.~\ref{subsec:perfmodel}) as well as a replica assignment for each job at each stage if it is assigned to the private cloud. The schedule also specifies which jobs are to be offloaded to the public cloud and at which stage. The scheduler loads this schedule text file. For each stage and replica, it determines the order in which jobs are to be executed using the start times from the schedule (for job stages assigned to the private cloud). 
The scheduler dispatches jobs for the first stage according to these sequence orders. On completion of a stage, the replica notifies the scheduler. The scheduler queues the job for the next stage, if one exists, where it again dispatches jobs according in the heuristics. 
%We note that  while the framework dispatches jobs to each replica in the scheduled order, it disregards the schedule start time for each job. Rather, it simply dispatches the next job as soon as the current job has completed.  We make this simplification because there is no  benefit, in terms of the makespan, to delaying a job, when the replica is available to process it, so long as the order of job executions is preserved. 
Intermediate data generated by a stage is stored in blob storage in the private cloud so it can be used in subsequent downstream stages. On completion of the last stage, the results of the job are also stored in the private cloud blob storage. 

With respect to the public cloud, serverless functions are pre-configured for each function in the application.
If at any stage, a job is scheduled to be executed in the public cloud, the scheduler subprocess corresponding to the stage offloads the stage to the public cloud i.e. executes the function corresponding to that stage in public cloud. This is achieved by uploading the input of that stage to blob storage in the public cloud. 
Multiple function stages can be offloaded by uploading to corresponding blob storage buckets in parallel.
The upload of this data triggers the execution of the corresponding serverless functions.   
Once a job starts executing in the public cloud, if the job is scheduled to complete all remaining stages in the public cloud, the scheduler has no other duty to perform for this job.  Any subsequent stages for that job are triggered by the storage of results in intermediate storage in the current stage. At the end of execution, the last stage in the public cloud, the public cloud function notifies the scheduler in the private cloud, which then downloads the results and stores them in private cloud blob storage. \sep{Explain what happens if later stages execute in the private cloud - I know we did not implement this, but describe it anyway} 


\subsection{Implementation} 
\sep{There is some redundancy in this subsection w.r.t. the previous subsection. It is fine for PSEG, but we may want to remove it for ICDCS.}
 In our prototype, for the public cloud environment, we use AWS Lambda to execute stages, and we use AWS S3 as a storage medium for inputs, intermediate storage, and results.  
%In AWS Lambda, each function instance runs in its own container and the developer can specify the memory configuration for these containers. Increasing memory configuration of a function allocates increased memory and proportional CPU to the instances of the function and thereby increases overall performance. According to our optimization problem definition, we setup the memory configuration of the AWS Lambda functions to a fixed memory, which gives a good price-performance benefit for our applications.}
To implement simple function chaining in AWS, we create a unique S3 bucket for each function to which the function writes its output data. We configure an AWS S3 trigger so that the writing of this intermediate data triggers the next lambda function in the chain. This next function reads its input data from the triggering S3 bucket.
If the scheduler dispatches multiple job stages to the public cloud, the AWS Lambda platform will scale to meet this demand by executing multiple copies of the required functions in parallel. For more complicated DAGs with parallel stages, we execute the pipeline using AWS Step Functions. The intermediate outputs are still stored in S3 buckets, however, once we trigger the first stage, Step functions will trigger the rest of the downstream Lambda functions on its own by passing \texttt{JSON} object between functions.

%\sep{Should we mention that we only use warm starts. Is this true? We can mention is/will provide a feature to eliminate cold starts, so our use of warm starts makes sense.} \das{Yes we use warm starts here. I am not entirely sure how to correctly and concisely mention AWS's new feature here so that they will understand. Also, I feel starting a discussion on warm and cold starts here opens a box of cans.} \sep{OK, we can ignore for PSEG, but we should address for ICDCS}


For the private cloud platform, we use  the popular open-source Function-as-a-Service vendor OpenFaaS. 
We deploy OpenFaaS on top of the Kubernetes Container Orchestration System \cite{kubernetes}
This private cloud is run on a server machine in our lab. %OpenFaaS supports serverless function execution as well as stateless microservice execution through the use of Docker and Kubernetes. 
When deploying serverless functions on OpenFaaS, the program creates a function that runs on a Kubernetes pod with an API address which, when invoked, executes the deployed function. 
%Scaling of such a function creates replicas in multiple pods which can be invoked via the same API. 
In a typical OpenFaaS deployment,  the load distribution to pods is handled by Kubernetes by default. Using L4 load balancing \cite{kubebalancing}, Kubernetes send function execution requests to pods depending on iptable rules via \textit{kube-proxy}. Each request is assigned to a pod in a  round robin fashion, and requests are queued at each pod until they can be processed.   
To implement our custom scheduler, we configure our prototype so that each pod runs exactly one function instance.
We create $I_k$ pods for each stage $k = 1 \ldots K$. Each pod is uniquely addressable via an \texttt{http} call.
Our scheduler uses these addresses to make requests (dispatch jobs) to specific replicas according to the schedule.
%This functionality allows us to implement our own scheduler that can invoke or make request to a specific replica of a function to execute a job.
%Since we assume that our infrastructure is fixed and resources are limited, this setting of individually addressable function replicas is is not much different from having a single addressible function with multiple replicas at the backend and thus provides a simplification to set up our scheduling problem. The advantage is that since we can now contact each function 'replica' uniquely via \texttt{http} calls, we can schedule jobs directly to a replica. 


%In Fig.~\ref{fig:openfaas},we describe our proposed architecture using a sample serverless application. 
%For ease of exposition, we consider an image processing application as an example, where a job consists of first rotating, then resizing and finally compressing an image. 

The details of the scheduler implementation are shown in Fig.~\ref{fig:openfaas}, for an application with two stages (Matrix Processing Application described in Sec~.\ref{apps.sec}) (Matrix Multiplication (MM), and LU decomposition (LU)).
A batch of job requests is submitted to the system through the OpenFaaS gateway. We then intercept the incoming requests via the custom scheduler module. The scheduler is  a long-running server process that is running as a function inside OpenFaaS. Jobs are submitted to the scheduler as \texttt{http} requests. 
The scheduler  has $N$ subprocesses, one for each function in the system. 

The subprocess corresponding to each function determines the sequencing of  jobs in that function and assigns jobs to the appropriate pods in the correct order. The subprocess also dispatches jobs to AWS Lambda in the public cloud when specified by the schedule. 
%There exists another handler subprocess which handles offloading tasks. This has a queue. Whenever a job is placed in the handler's queue, it uploads the image/matrix corresponding to that job to the S3 bucket from local Minio storage. For multiple jobs, this handler can resume parallel uploads via multithreading.}
For job stages that are executed in the private cloud, the  function's subprocess forwards the request to the specified pod via an asynchronous calls through the NATS Streaming queue already present in OpenFaaS. 
%Subsequently, a Queue worker dequeues request from the NATS queue and invokes the function replica with that request.
When a replica completes execution of the function, it uploads the results to a local blob storage, which is implemented using Minio~\cite{minio}. The replica then notifies the scheduler via an \texttt{http} \texttt{POST} request, so the scheduler can dispatch the job to any subsequent function(s), per the schedule. 
%The Queue workers in the Fig.~\ref{fig:openfaas} has the job of dequeuing jobs/requests from the NATS queue and invoking a correct function replica with that request. A queue worker is blocked as long as the replica is executing, hence for increased parallelism we would need many queue workers.}
%It is to be noted that, as per our optimization problem \ref{objective.eq}, we design the scheduler such that it allows execution of one job at a time at each replica of any function at any given time. 
For job stages that are scheduled to be executed in the public cloud, the corresponding data is uploaded by a separate handler process, which uploads data for multiple jobs in parallel as necessary.

For jobs that are executed in the public cloud, the result of each function execution is stored in AWS S3. 
The last function in the pipeline, when completes, notifies the scheduler, which then downloads the results from S3 to a private Minio bucket.
%On completion of the last function for a job in AWS Lambda, a \texttt{http} request is made to the scheduler to inform it of completion. We then transfer the  results from the public cloud to the private cloud, using a separate downloader system that is triggered whenever new the previously mentioned \texttt{http} call is received.
For each job, this process continues until all the functions have executed. 


%\begin{figure}[htpb]
%    \centering
%    \includegraphics[scale=.27]{Images/POds.png}
%    \caption{Scheduler Implementation.} \label{fig:openfaas}
%\end{figure}
